Centralized vs. Decentralized Security for Space AI Systems? A New Look

This paper investigates the trade-off between centralized and decentralized security management in constellations of satellites to balance security and performance. We highlight three key AI architectures for automated security management: (a) centralized, (b) distributed and (c) federated. The centralized architecture is the best option short term, providing fast training, despite the hard challenge of the communication latency overhead across space. Decentralized architectures are better alternatives in the longer term, providing enhanced scalability and security.

==> trame.tex <==
Le domaine spatial ou « New Space » est une nouvelle frontière pour les télécoms et l’avenir du cloud : défis opérateurs (e.g., constellations de satellites, space cloud computing), acteurs multiples, contraintes fortes sur les communications (e.g., latence, bande passante, mobilité, confiance, résilience), nombreuses menaces [1][3]. Comment sécuriser ces systèmes distribués de l’extrême ? [6].
L’isolation est un défi sécurité critique en environnement multi-locataires (« multi-tenant » en anglais), extension à l’espace des risques des infrastructures terrestres cloud, centralisées ou décentralisées.  Quel impact pour des violations d’isolation, e.g., défaut d’intégrité des données en environnement virtualisé ou brèche du système d’IA ? Avec quelles conséquences pour le système réel (e.g., collisions de satellites, déni de service) ? Quelles contre-mesures pour limiter ces risques ? Comment les placer au mieux, e.g., de manière automatisée, sur terre et dans l’espace ?
4. ANALYSE DE L‘EXISTANT (quelles sont les méthodes existantes pour répondre à cette problématique ? quelles sont leurs limites ? – cette description doit contenir des références) - 10 lignes
Au niveau du continuum cloud-to-space, des voies prometteuses en mode cloud ou edge combinent : 1) réalité étendue (XR) pour explorer la sécurité dans un environnement contrôlé et flexible, jumeau numérique du système spatial, mais sans disposer des contraintes du milieu spatial qui rendent complexes ou coûteuses le déploiement direct de nouvelles contre-mesures [2] ; 2) IA et grands modèles de langages (LLMs) pour plus de dynamisme, e.g., pour visualiser les vulnérabilités et automatiser le placement de contre-mesures [7][9][16]. Malheureusement, ces approches introduisent des risques nouveaux : 1) au niveau cloud, pour les systèmes virtuels partagés multi-utilisateurs [4], les vulnérabilités de l’environnement virtuel ont un impact sur la sûreté des environnements physiques ; 2) à l’edge, dans les environnements de perception coopérative pour véhicules connectés, on trouve de nouvelles vulnérabilités liées à l’IA avec un impact similaire [5].
5. PROPOSITION SCIENTIFIQUE DU STAGE (quelles pistes scientifiques seront envisagées dans le stage ? en quoi cette approche est-elle innovante par rapport à l’existant ? – cette description doit contenir des références) - minimum 10 lignes
Avec l’essor du New Space [1][2]|10]|11][13] et d’un continuum device/edge/cloud/space [8][12], on étudiera les solutions existantes pour l’isolation multi-locataires pour les infrastructures spatiales de type constellations de satellites [3][6]|7][9], environnements virtuels partagés [4] et systèmes de véhicules connectés [5] pour en déduire des exigences de sécurité pour l’isolation des données.  
On proposera une architecture générique d’isolation des données pour l’IA pour un système de jumeau numérique général augmenté de contre-mesures adéquates. L’IA [7][9][16] pourra concerner le jumeau numérique lui-même, l’interface entre le système spatial et sa réplique cloud, le placement des contre-mesures, ou l’équilibrage entre plusieurs tiers (espace, cloud, edge), e.g., en utilisant des d’algorithmes d’apprentissage fédérés [14] ou décentralisés [15]. On implantera un prototype simple de jumeau numérique (e.g., à l’aide du système Unity ou d’autres simulateurs de réalité augmentée) et on analysera les contre-mesures applicables (e.g., d’isolation matérielle [17]).
Dans un second temps, on raffinera sur un cas d’usage l’architecture générale définie, par exemple pour la perception coopérative pour les systèmes de véhicules connectés ou pour le cloud distribué entre environnements terrestres et spatiaux. On évaluera le prototype réalisé en termes de sécurité, privacy et enseignements applicables au cas d’usage et transposables aux environnements spatiaux. On aura l’opportunité de publier les résultats de recherche obtenus dans des conférences spécialisées.
6. RESULTATS ATTENDUS (quelle est la nature des résultats attendus ? comment seront-ils évalués ?) - 5 lignes
1.	On explorera les défis d’isolation multi-locataires du New Space (e.g., IA décentralisée, isolation d’espaces virtuels partagés ou de systèmes de perception collaborative véhiculaires).
2.	On proposera une architecture de sécurité pour système XR+IA multi-locataires, jumeau numérique d’un système de télécom spatial et on en réalisera un prototype
3.	On l’évaluera sur un cas d’usage en termes de sécurité, performance et flexibilité.

